Long Sequence Decoder Network for Mobile Sensing

The reconstruction and estimation of spatio-temporal patterns poses significant challenges when sensor measurements are limited. The use of mobile sensors adds additional complexity due to the change in sensor locations over time. In such cases, historical measurement and sensor information are useful for better performance, including models such as Kalman filters, recurrent neural networks (RNNs) or transformer models. However, many of these approaches often fail to efficiently handle long sequences of data in such scenarios and are sensitive to noise. In this paper, we consider a model-free approach using the {\em structured state space sequence} (S4D) model as a deep learning layer in traditional sequence models to learn a better representation of historical sensor data. Specifically, it is integrated with a shallow decoder network for reconstruction of the high-dimensional state space. We also introduce a novel initialization of the S4D model using a Butterworth filter design to reduce noise in the inputs. Consequently, we construct a robust S4D (rS4D) model by appending the filtering S4D layer before the original S4D structure. This robust variant enhances the capability to accurately reconstruct spatio-temporal patterns with noisy mobile sensor measurements in long sequence. Numerical experiments demonstrate that our model achieves better performance compared with previous approaches. Our results underscore the efficacy of leveraging state space models within the context of spatio-temporal data reconstruction and estimation using limited mobile sensor resources, particularly in terms of long-sequence dependency and robustness to noise.

==> notes.tex <==
\section{Method}

\subsection{State Space Models}

What is a state space model? How does it compare to an LSTM?

Consider the 1-dimentional input-output, continuous-time time-invariant system:
\begin{equation}
\begin{split}
    \mathbf{x}'(t) &= \mathbf{A} \mathbf{x}(t) + \mathbf{B} \mathbf{u}(t) \\
    \mathbf{y}(t) &= \mathbf{C} \mathbf{x}(t)
\end{split}
\end{equation}
where $\mathbf{u}(t), \mathbf{y}(t) \in \mathbb{R}$, so $\mathbf{B} \in \mathbb{R}^{N \times 1}$ and $\mathbf{C} \in \mathbb{R}^{1 \times N}$.

The general state-space model does not work well in practice, possibly because the exponential solution to the continuous-time system suffers from gradient vanishing/exploding in a long sequence.

However, they leverage the HiPPO theory of continuous-time memorization, which refers to a class of matrices that can memorize the history of input $\mathbf{u}(t)$ in the state $\mathbf{x}(t)$.
(TODO: more info on HiPPO theory)

In particular, a specific HiPPO matrix is defined as follows:
\begin{equation}
    \mathbf{A}_{nk} = -
    \begin{cases}
        (2n+1)^{1/2} (2k+1)^{1/2} & n > k \\
        n+1 & n = k \\
        0 & n < k
    \end{cases}
\end{equation}

\textbf{The rest of the work discusses the setup on a computational level.}

In order to efficiently compute the solution of the state space model. In order to do so, a discrete convolutional representation is considered, and the convolution kernel should be fast to compute. 

The HiPPO matrix itself does not produce simple kernel computations. The work solves this issue using the following thinking:
\begin{itemize}
    \item The original matrix is normal-plus-low-rank (NPLR), therefore it can be conjugated into diagonal-plus-low-rank (DPLR) form;
    \item Compute the kernel using its generation function and inverse FFT instead of direct calculation;
    \item Use Woodbury matrix inverse identity to reduce the inverse of a DPLR matrix in terms of the inverse of the diagonal part;
    \item Compute Cauchy kernel of the diagonal form;
\end{itemize}

First, we show that the HiPPO matrix is NPLR. Specifically, we have 
\begin{equation}
    \mathbf{A}_{nk} + \frac{1}{2} \sqrt{(2n+1)(2k+1)} = -
    \begin{cases}
        \frac{1}{2} (2n+1)^{1/2} (2k+1)^{1/2} & n > k \\
        \frac{1}{2} & n = k \\
        -\frac{1}{2} (2n+1)^{1/2} (2k+1)^{1/2} & n < k
    \end{cases}.
\end{equation}
Therefore, in matrix form,
\begin{equation}
    \mathbf{A} + \mathbf{P}\mathbf{P}^\top = -\frac{1}{2} \mathbf{I} + \mathbf{S},
\end{equation}
where $\mathbf{P}_n = \sqrt{\frac{2n+1}{2}}$ is rank 1 and $\mathbf{S}_{nk} = \begin{cases}
        -\frac{1}{2} (2n+1)^{1/2} (2k+1)^{1/2} & n > k \\
        0 & n = k \\
        \frac{1}{2} (2n+1)^{1/2} (2k+1)^{1/2} & n < k
\end{cases}$ 
is skew-symmetric that is diagonalizable by a unitary matrix $\mathbf{V}$, $\mathbf{S} = \mathbf{V}\mathbf{\Lambda} \mathbf{V}^*$. Then,
\begin{equation}
\begin{split}
    \mathbf{A} &= -\frac{1}{2} \mathbf{I} + \mathbf{S} - \mathbf{P}\mathbf{P}^\top \\
    &= \mathbf{V} (\mathbf{\Lambda} -\frac{1}{2} \mathbf{I}) \mathbf{V}^* - \mathbf{P}\mathbf{P}^\top \\
    &= \mathbf{V} (\mathbf{\Lambda} -\frac{1}{2} \mathbf{I} - (\mathbf{V}^*\mathbf{P})(\mathbf{V}^*\mathbf{P})^*) \mathbf{V}^* 
\end{split}
\end{equation}

As a result, the original SSM model $(\mathbf{A}, \mathbf{B}, \mathbf{C})$ can be transformed into $(\mathbf{V}^{-1}\mathbf{A}\mathbf{V} = \mathbf{\Lambda} -\frac{1}{2} \mathbf{I} - (\mathbf{V}^*\mathbf{P})(\mathbf{V}^*\mathbf{P})^*, \mathbf{V}^{-1}\mathbf{B}, \mathbf{C}\mathbf{V})$. The new system dynamics is DPLR. And from now on, we assume that the SSM model is DRLR with $\mathbf{A} = \mathbf{\Lambda} - \mathbf{P}\mathbf{Q}^*$. 

Next, the continuous-time SSM can be discretized using the bilinear method for a step size $\triangle$. 
\begin{equation}
    \begin{split}
    \mathbf{x}_k &= \overline{\mathbf{A}} \mathbf{x}_{k-1} + \overline{\mathbf{B}} \mathbf{u}_k, \\
    \mathbf{y}_k &= \overline{\mathbf{C}} \mathbf{x}_k, \\
    \overline{\mathbf{A}} &= (\mathbf{I} - \triangle/2 \cdot \mathbf{A})^{-1}  (\mathbf{I} + \triangle/2 \cdot \mathbf{A}), \\
    \overline{\mathbf{B}} &= (\mathbf{I} - \triangle/2 \cdot \mathbf{A})^{-1} \triangle \mathbf{B}, \quad \overline{\mathbf{C}} = \mathbf{C}.
\end{split}
\end{equation}

Using Woodbury's identity on the first component of $\overline{\mathbf{A}}$, we can show that it is a product of two DPLR matrices, and the matrix-vector operation can be performed in $\mathcal{O}(N)$. 

In convolution form, the SSM can also be vectorized into $\mathbf{y} = \overline{\mathbf{K}} \ast \mathbf{u}$, $\overline{\mathbf{K}} = (\overline{\mathbf{C}}\overline{\mathbf{B}}, \overline{\mathbf{C}}\overline{\mathbf{A}}\overline{\mathbf{B}}, \cdots, \overline{\mathbf{C}}\overline{\mathbf{A}}^{L-1}\overline{\mathbf{B}})$. 
Directly computing the kernel requires computing $\overline{\mathbf{A}}^{L-1}$, which is not simple even when $\overline{\mathbf{A}}$ is DPLR.
The work thus propose to first use the generating function and then apply the inverse FFT to compute the kernel function. 
The generating function at node $z$ is defined as $\hat{\mathbf{K}} (z) = \sum_{i=0}^{L-1} \overline{\mathbf{C}}\overline{\mathbf{A}}^i\overline{\mathbf{B}}z^i = \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L z^L)(I - \overline{\mathbf{A}} z)^{-1} \overline{\mathbf{B}}$, and the generating function at nodes $\Omega$ is $\hat{\mathbf{K}} (\Omega) = (\hat{\mathbf{K}} (\omega))_{\omega \in \Omega}$. 
Computed at the roots of unity $\Omega = \{\exp(-2\pi i \frac{k}{L}: k \in [L])\}$, $\hat{\mathbf{K}} := \hat{\mathbf{K}} (\Omega)$ is the Discrete Fourier Transform (DFT) of $\overline{\mathbf{K}}$.

At any root of unity $z$, the generation function can be written as 
\begin{equation}
\begin{split}
    \hat{\mathbf{K}}(z) &= \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L)(I - \overline{\mathbf{A}} z)^{-1} \overline{\mathbf{B}} \\
    &= \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L)\left( (\mathbf{I} - \frac{\triangle}{2} \mathbf{A})^{-1}(\mathbf{I} - \frac{\triangle}{2} \mathbf{A}) - (\mathbf{I} - \frac{\triangle}{2} \mathbf{A})^{-1} (\mathbf{I} + \frac{\triangle}{2} \mathbf{A}) z \right)^{-1} \overline{\mathbf{B}} \\
    &= \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L)\left( (\mathbf{I} - \frac{\triangle}{2} \mathbf{A}) - (\mathbf{I} + \frac{\triangle}{2} \mathbf{A}) z \right)^{-1} (\mathbf{I} - \frac{\triangle}{2} \mathbf{A})\overline{\mathbf{B}} \\
    &= \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L)\left((1-z) \mathbf{I} - \frac{\triangle}{2} (1+z) \mathbf{A} \right)^{-1} \triangle \mathbf{B} \\
    &= \frac{2}{1+z} \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L) \left(\frac{2}{\triangle} \frac{1-z}{1+z} \mathbf{I} - \mathbf{A} \right)^{-1} \mathbf{B} \\
    &= \frac{2}{1+z} \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L) \left(\frac{2}{\triangle} \frac{1-z}{1+z} \mathbf{I} - \mathbf{\Lambda} + \mathbf{P}\mathbf{Q}^* \right)^{-1} \mathbf{B} \\
    &= \frac{2}{1+z} \left[ \Tilde{\mathbf{C}} \mathbf{R}(z) \mathbf{B} - \Tilde{\mathbf{C}} \mathbf{R}(z)\mathbf{P} (1 + \mathbf{Q}^*\mathbf{R}(z)\mathbf{P})^{-1} \mathbf{Q}^*\mathbf{R}(z) \mathbf{B} \right]
\end{split}
\end{equation}
$\Tilde{\mathbf{C}} := \overline{\mathbf{C}}(I - \overline{\mathbf{A}}^L)$ can be learned directly by reparameterization instead of $\mathbf{C}$. $\mathbf{R}(z) := (\frac{2}{\triangle} \frac{1-z}{1+z} \mathbf{I} - \mathbf{\Lambda})^{-1}$ and its product operations can be computed efficiently by Cauchy kernel numerically. 

\subsection{S4 block}

The structure of the S4 block is then set up as follows. 
A separate state-space model with 1D input and output is considered for each feature element in the multi-dimensional feature input. 
A DPLR dynamics is used, so $\mathbf{A} = \text{diag}(\mathbf{a}) - \mathbf{p}\mathbf{p}^*, \mathbf{a},\mathbf{p} \in \mathbb{R}^N$. 
Along with $\mathbf{b}, \mathbf{c} \in \mathbb{R}^N$ , they make up of the parameters in a S4 block. 
The low rank component can be more generally expressed more generally as  $\mathbf{p}\mathbf{q}^*$ with separate vectors, but it suffers from numerical instability~\cite{goel2022s}.
Additionally, the output can have multiple values in the form of channels, so $\mathbf{C} \in \mathbb{R}^{C \times N}$. 
The parameters are initialized as the HIPPO matrix. 

Suppose we have a feature input of size $H$. 
S4 handles multiple features by simply defining $H$ independent copies of the state-space model, and then mixing the $CH$ outputs with a position-wise linear layer.
The total number of parameters in a S4 layer is $O(CHN) + O(CH^2)$. 

\subsection{S4D block}

Instead of using a DPLR matrix, the dynamics matrix is diagonal, with its initialization being the diagonal component of HIPPO matrix decomposition.
Gu et al.~\cite{gu2022parameterization} further discusses other forms of initialization.
This change into diagonal matrix enables further simplification in the calculation of the kernel, and opens up new possibility of discretization method of the continuous dynamics. 
Specifically, we can write the kernel as a Vandermonde matrix-vector multiplication.
The resulting discrete convolution kernel depends only on the element-wise product $\mathbf{B} \circ \mathbf{C}_i$ for each channel $i$ of $\mathbf{C}$. 
Therefore, we can train just on $\mathbf{C}$ while keeping $\mathbf{B}=1$ constant.
However, Gu et al.~\cite{gu2022parameterization} show from experiments that training $\mathbf{B}$ and $\mathbf{C}$ independently gives minor but consistent improvement in performance. 

This also releases the model from the discritization requirement from previous models due to computation complexity. 
Discritizations such as zero-order hold (ZOH) and bilinear can be more efficiently computed on the diagonal model. 

\subsection{S4DC block}

The theoretical guidance provided by HiPPO matrix is only in effect at the initialization stage. 
The S4(D) structure is updated freely afterwards during training. 
We want to use characteristics of the state-space model to further improve model training. 

The $H_2$ norm of a system measures system sensitivity to white noise input.
It is the average output gain over all frequencies of the input, which is minimized in optimal control.
The $H_2$ norm can be defined with respect to the transfer function $\hat{G}(s) = \mathbf{C} (s\mathbb{I} - \mathbf{A})^{-1} \mathbf{B}$,
\begin{equation}
    \|\hat{G}\|_2^2 = \frac{1}{2\pi} \int_{-\infty}^\infty \text{tr}(\hat{G}(j\omega)^* \hat{G}(j\omega)) d\omega.
\end{equation}
By the Plancherel theorem, it is equivalent to the time-domain norm of the impulse response (convolution kernel) function 
$H(\tau) = \begin{cases}
    \mathbf{C} e^{\mathbf{A}\tau} \mathbf{B} & \tau \ge 0 \\
    0 & \tau < 0 
\end{cases}$,
\begin{equation}
    \|G\|_2^2 = \|H\|_2^2 = \int_0^\infty \text{tr}(\mathbf{C} e^{\mathbf{A}t} \mathbf{B}\mathbf{B}^* e^{\mathbf{A}^*t} \mathbf{C}^*) dt.
\end{equation}

Applying to the S4D model, we have:
\begin{equation}
\begin{split}
    \|G\|_2^2 &= \int_0^\infty \sum_{i=1}^N \sum_{j=1}^N \mathbf{c}_i\overline{\mathbf{c}_j} \mathbf{b}_i \overline{\mathbf{b}_j} e^{(\mathbf{a}_i + \overline{\mathbf{a}_j})t} dt \\
    &= \sum_{i=1}^N \sum_{j=1}^N \int_0^\infty \mathbf{c}_i\overline{\mathbf{c}_j} \mathbf{b}_i \overline{\mathbf{b}_j} e^{(\mathbf{a}_i + \overline{\mathbf{a}_j})t} dt \\
    &= \sum_{i=1}^N \sum_{j=1}^N -\frac{\mathbf{c}_i\overline{\mathbf{c}_j} \mathbf{b}_i \overline{\mathbf{b}_j} }{\mathbf{a}_i + \overline{\mathbf{a}_j}} \\
    &= \mathbf{X}^* \mathbf{M} \mathbf{X},
\end{split}
\end{equation}
where $\mathbf{X}_i = \mathbf{B} \circ \mathbf{C}_i$, and $\mathbf{M}_{ij} = -\frac{1}{\mathbf{a}_i+\overline{\mathbf{a}_j}}$.
$\mathbf{M}$ is Hermitian and positive definite, so its eigenvalues are all positive. 
Therefore, assuming $\mathbf{X}$ has norm 1, then the $H_2$ system norm is minimized when $\mathbf{X}$ is the eigenvector corresponding to the smallest eigenvalue of $\mathbf{M}$. 
Then, $\|G\|_2^2 = \lambda_{\min}(\mathbf{M})$. 
In general, the solution $\mathbf{X}$ is not unique and the eigenvectors are subtract to a factor of $e^{i\phi}, \phi \in \mathbb{R}$ for complex solutions. 
To impose uniqueness and convergence to the solution, we can constraint the phase of the eigenvector such that the first element lies on the positive real axis.

When $\mathbf{C}$ has multiple output channels, the output energy becomes $\|G\|_2^2 = \text{tr} (\mathbf{X}^* \mathbf{M} \mathbf{X})$. 
Under the constraint that $\mathbf{X}$ is orthogonal, $\mathbf{X}^* \mathbf{X} = \mathbf{I}$, the solution is the eigenvectors corresponding to the smallest $C$ eigenvalues, and $\|G\|_2^2 = \sum_{i=1}^C \lambda_{-i}(\mathbf{M})$. 

There is no closed-form solution of eigenvalue and eigenvector pairs of the matrix. 
Power iteration is a simple iterative approach to find the largest (in absolute value) eigenvalue and eigenvector of a matrix. 
Here, we use a shifted power iteration to find the eigenvector corresponding to the smallest eigenvalue of $\mathbf{M}$.
Since $\mathbf{M}$ is positive definite, and $\|\mathbf{M}\|_2 \leq \|\mathbf{M}\|_F$, then the smallest (in absolute value) eigenvalue and eigenvector of $\mathbf{M}$ is equivalent to the largest (in absolute value) eigenvalue and eigenvector of $\mathbf{M} - \|\mathbf{M}\|_F \mathbf{I}$.
An additional step is needed to ensure that $\mathbf{X}$ has orthogonal columns. 
This orthogonlization can be done using QR decomposition.

\begin{algorithm}
\caption{Orthogonalized shifted power iteration}
\KwIn{$\mathbf{X}$, $\mathbf{M}$, number of iterations $T$}
\KwOut{$\mathbf{X}_T$}
Initialize $\mathbf{X}_0 =  \mathbf{X}$ and shifted matrix $\tilde{\mathbf{M}} = \mathbf{M} - \|\mathbf{M}\|_F \mathbf{I}$\;
\For{$t=[0,T-1]$}{
    $\tilde{\mathbf{X}}_{t+1} = \tilde{\mathbf{M}} \mathbf{X}_t$\;
    $\mathbf{X}_{t+1}, \_ = QR(\tilde{\mathbf{X}}_{t+1})$\;
}

\end{algorithm}

% We keep track of $\mathbf{X}$ instead of $\mathbf{C}$ as a variable in the model, which can be retrieved easily with $\mathbf{C} = \mathbf{X} \oslash \mathbf{B}$. 
Theoretically, since the convolution kernel only depends on $\mathbf{X}$, we no longer need to keep trainable copies of $\mathbf{B}$ or $\mathbf{C}$. 
However, since the previous work allows $\mathbf{B}$ to be either fixed or trainable and has reported better performance with training $\mathbf{B}$, we do the same.

\begin{algorithm}
\caption{Training Step}
\SetKwInOut{Parameter}{Parameter}
\Parameter{$\mathbf{A}$, $\mathbf{B}$, $\mathbf{X}$}
Compute $\mathbf{C} = \mathbf{X} \oslash \mathbf{B}$\;
Fit data using $\mathbf{A}$, $\mathbf{B}$, and $\mathbf{X}$, and update $\mathbf{A}$, $\mathbf{B}$ through back-propagation\;
Compute $\mathbf{M}$ from $\mathbf{A}$\;
Perform one step of shifted power iteration with $\mathbf{X}$, $\mathbf{X} = (\mathbf{M} - \|\mathbf{M}\|_F \mathbf{I}) \mathbf{X}$\;
Normalize $\mathbf{X}$\;
\end{algorithm}


\subsection{S4Decoder}

We put the S4 blocks with a shallow decoder network. 
